Be Like Water: Robustness to Extraneous Variables Via Adaptive Feature Normalization

Extraneous variables are variables that are irrelevant for a certain task, but heavily affect the distribution of the available data. In this work, we show that the presence of such variables can degrade the performance of deep-learning models. We study three datasets where there is a strong influence of known extraneous variables: classification of upper-body movements in stroke patients, annotation of surgical activities, and recognition of corrupted images. Models trained with batch normalization learn features that are highly dependent on the extraneous variables. In batch normalization, the statistics used to normalize the features are learned from the training set and fixed at test time, which produces a mismatch in the presence of varying extraneous variables. We demonstrate that estimating the feature statistics adaptively during inference, as in instance normalization, addresses this issue, producing normalized features that are more robust to changes in the extraneous variables. This results in a significant gain in performance for different network architectures and choices of feature statistics.

==> tables_tex/CIFAR10c.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\begin{tabular}[c]{}\end{tabular}} & \multicolumn{6}{c|}{Absolute Accuracy Values}                          & \multicolumn{6}{c|}{Drop in Accuracy Relative to CIFAR10}              \\ \cline{2-13} 
                                                                                    & \multicolumn{2}{c|}{Non-Adaptive} & \multicolumn{4}{c|}{Adaptive}      & \multicolumn{2}{c|}{Non-Adaptive} & \multicolumn{4}{c|}{Adaptive}      \\ \cline{2-13} 
                                                                                    & BN            & FRN(Batch)        & IN    & FRN   & BN    & FRN(Batch) & BN            & FRN(Batch)        & IN    & FRN   & BN    & FRN(Batch) \\ \hline
\textbf{CIFAR10}                                                                    & 94.15         & 91.44             & 92.08 & 90.99 & 91.48 & 87.47      &               &                   &       &       &       &            \\ \hline
brightness                                                                          & 92.09         & 89.25             & 91.07 & 89.87 & 90.57 & 85.74      & 2.06          & 2.19              & 1.01  & 1.12  & 0.91  & 1.73       \\ \hline
contrast                                                                            & 75.97         & 70.04             & 91.62 & 88.48 & 88.66 & 84.1       & 18.18         & 21.4              & 0.46  & 2.51  & 2.82  & 3.37       \\ \hline
defocus\_blur                                                                       & 76.78         & 77.3              & 87.51 & 87.03 & 89.88 & 86.39      & 17.37         & 14.14             & 4.57  & 3.96  & 1.6   & 1.08       \\ \hline
elastic\_transform                                                                  & 79.44         & 78.25             & 84.19 & 83.91 & 83.36 & 79.93      & 14.71         & 13.19             & 7.89  & 7.08  & 8.12  & 7.54       \\ \hline
fog                                                                                 & 84.59         & 81.0              & 88.02 & 86.15 & 88.46 & 84.58      & 9.56          & 10.44             & 4.06  & 4.84  & 3.02  & 2.89       \\ \hline
frost                                                                               & 73.44         & 69.99             & 83.65 & 81.86 & 80.54 & 73.4       & 20.71         & 21.45             & 8.43  & 9.13  & 10.94 & 14.07      \\ \hline
gaussian\_blur                                                                      & 63.95         & 67.63             & 84.34 & 84.66 & 89.79 & 85.84      & 30.2          & 23.81             & 7.74  & 6.33  & 1.69  & 1.63       \\ \hline
gaussian\_noise                                                                     & 50.32         & 48.62             & 67.65 & 63.85 & 69.89 & 67.17      & 43.83         & 42.82             & 24.43 & 27.14 & 21.59 & 20.3       \\ \hline
glass\_blur                                                                         & 51.43         & 48.34             & 64.25 & 62.49 & 65.54 & 64.68      & 42.72         & 43.1              & 27.83 & 28.5  & 25.94 & 22.79      \\ \hline
impulse\_noise                                                                      & 59.65         & 61.23             & 73.26 & 72.43 & 72.28 & 68.52      & 34.5          & 30.21             & 18.82 & 18.56 & 19.2  & 18.95      \\ \hline
jpeg\_compression                                                                   & 77.96         & 78.77             & 79.32 & 79.61 & 76.04 & 75.61      & 16.19         & 12.67             & 12.76 & 11.38 & 15.44 & 11.86      \\ \hline
motion\_blur                                                                        & 73.65         & 70.25             & 86.27 & 86.42 & 86.74 & 82.9       & 20.5          & 21.19             & 5.81  & 4.57  & 4.74  & 4.57       \\ \hline
pixelate                                                                            & 69.1          & 68.15             & 79.48 & 82.94 & 83.51 & 80.45      & 25.05         & 23.29             & 12.6  & 8.05  & 7.97  & 7.02       \\ \hline
saturate                                                                            & 90.44         & 87.47             & 89.93 & 87.69 & 90.29 & 85.64      & 3.71          & 3.97              & 2.15  & 3.3   & 1.19  & 1.83       \\ \hline
shot\_noise                                                                         & 61.58         & 58.73             & 72.21 & 69.48 & 73.89 & 70.97      & 32.57         & 32.71             & 19.87 & 21.51 & 17.59 & 16.5       \\ \hline
snow                                                                                & 78.78         & 74.88             & 84.35 & 82.8  & 79.72 & 73.52      & 15.37         & 16.56             & 7.73  & 8.19  & 11.76 & 13.95      \\ \hline
spatter                                                                             & 83.94         & 81.81             & 86.69 & 85.3  & 84.12 & 79.47      & 10.21         & 9.63              & 5.39  & 5.69  & 7.36  & 8.0        \\ \hline
speckle\_noise                                                                      & 64.81         & 61.54             & 72.18 & 70.3  & 73.99 & 70.78      & 29.34         & 29.9              & 19.9  & 20.69 & 17.49 & 16.69      \\ \hline
zoom\_blur                                                                          & 70.97         & 71.06             & 84.08 & 84.68 & 88.49 & 84.98      & 23.18         & 20.38             & 8.0   & 6.31  & 2.99  & 2.49       \\ \hline
\textbf{Average}                                                                    & 72.57         & 70.75             & 81.58 & 80.52 & 81.88 & 78.14      & 21.58         & 20.69             & 10.5  & 10.47 & 9.6   & 9.33       \\ \hline
\end{tabular}

==> tables_tex/normalization_components.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Normalization\\ Scheme\end{tabular}}                            & \textbf{\begin{tabular}[c]{@{}c@{}}Moments \end{tabular}}                   & \textbf{\begin{tabular}[c]{@{}c@{}}Batch size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Adaptive during \\ inference?\end{tabular}} \\ \hline
Batch normalization (BN)                                                                           & \begin{tabular}[c]{@{}c@{}}Mean and \\ standard deviation \end{tabular} & \begin{tabular}[c]{@{}c@{}} \textgreater 1 \end{tabular}            & No                                                                             \\ \hline
\begin{tabular}[c]{@{}c@{}}Batch Feature Response \\ Normalization (BFRN)\end{tabular}             & Mean square                                                                     & \begin{tabular}[c]{@{}c@{}}\textgreater 1\end{tabular}            & No                                                                             \\ \hline
Instance Normalization (IN)                                                                        & \begin{tabular}[c]{@{}c@{}}Mean and \\standard deviation\end{tabular} & 1                                                                                                    & Yes                                                                            \\ \hline
\begin{tabular}[c]{@{}c@{}}Feature Response \\ Normalization (FRN)\end{tabular}                    & Mean square                                                                     & 1                                                                                                    & Yes                                                                            \\ \hline
\begin{tabular}[c]{@{}c@{}}Batch Normalization \\ (Adaptive)(BNa)\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}Mean and \\standard deviation\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textgreater 1\end{tabular}            & Yes                                                                            \\ \hline
\begin{tabular}[c]{@{}c@{}}Batch Feature Response \\ Normalization (Adaptive) (BFRNa)\end{tabular} & Mean squares                                                                    & \begin{tabular}[c]{@{}c@{}}\textgreater 1\end{tabular}            & Yes                                                                            \\ \hline
\end{tabular}

